Blockchain Censorship

Permissionless blockchains promise to be resilient against censorship by a single entity. This suggests that deterministic rules, and not third-party actors, are responsible for deciding if a transaction is appended to the blockchain or not. In 2022, the U.S. Office of Foreign Assets Control (OFAC) sanctioned a Bitcoin mixer and an Ethereum application, putting the neutrality of permissionless blockchains to the test. In this paper, we formalize quantify and analyze the security impact of blockchain censorship. We start by defining censorship, followed by a quantitative assessment of current censorship practices. We find that 46% of Ethereum blocks were made by censoring actors that intend to comply with OFAC sanctions, indicating the significant impact of OFAC sanctions on the neutrality of public blockchains. We further uncover that censorship not only impacts neutrality, but also security. We show how after Ethereum's move to Proof-of-Stake (PoS) and adoption of Proposer-Builder Separation (PBS) the inclusion of censored transactions was delayed by an average of 85%. Inclusion delays compromise a transaction's security by, e.g., strengthening a sandwich adversary. Finally we prove a fundamental limitation of PoS and Proof-of-Work (PoW) protocols against censorship resilience.

==> censorship_definition_fork.tex <==
\section{Censorship}\label{sec:censorship}

\subsection{System Model}\label{sec:system}
In the following we define this work's system model. We focus on a single blockchain $\blockchain$, where the term block\emph{chain} is used for simplicity and can equally refer to a block Directed Acyclic Graph (DAG)~\cite{lewenberg2015inclusive}. A blockchain user $u$ can create multiple addresses $a_i$ with their wallet. The user can then sign and issue a transaction $tx_a$ from an address $a$, by sending the transaction to one of the operators participating in $\blockchain$'s network (e.g. a blockchain node, a public RPC provider that is not a node, or a block builder). For brevity, we will use the term ``validator'' to refer both to validators and to miners whenever the choice of a consensus mechanism is not important. Once the transaction $tx_a$ reaches a validator, $tx_a$ can be included in a block $b$ added to $\blockchain$. We assume that the validator is not restricted by $\blockchain$'s consensus mechanism in their choice which transactions to include in a block and how to order transactions in that block.

\subsection{Censorship Within a Blockchain, Not of a Blockchain}\label{sec:scope}
``Blockchain censorship'' may be understood to refer both to censorship that takes place within a blockchain (against selected users, transactions, blocks) and to censorship targeted at an entire blockchain network. In this work, we focus on the former, but we wish to note that ineffectiveness of attempts by state actors to achieve censorship within a blockchain (e.g., targeting specific blockchain users who are subject to economic sanctions), may lead to attempts at censorship of entire blockchains. This could involve legal prohibitions on participation in and on providing services (including, e.g., internet access services) to a blockchain network.

\subsection{Definitions}\label{sec:def}

\subsubsection{Previous definitions}\label{sec:prevdef}
In previous work on censorship and censorship resistance on blockchains, ``censorship'' has been understood as:
\begin{itemize}
  \item excluding from the blockchain an included, but not finalized block~\cite{thin2018formal,silva2020impact}, e.g., by \emph{feather forking}~\cite{zhang2019lay};
  \item not including in a block a transaction targeted by censorship~\cite{silva2020impact,crain2021red};
  \item rejecting consensus messages from a validator targeted by censorship~\cite{xian2019improved}.
\end{itemize}
The first kind of exclusion may be due to the contents of a transaction the block contains (including, e.g., its sender and addressee) or because of who mined (proposed) the block~\cite{thin2018formal}. Exclusion of the second kind may similarly be due to the contents of the transaction or the identity of a user associated with it.

Notably, it is standard to distinguish \emph{censorship} from \emph{re-ordering} of transactions~\cite{buterin2021sok,qin2022quantifying,chitra2022improving,auer2022miners}. Censorship has not been considered to refer to block builders ordering (``re-ordering'') transactions in a block in a different way than expected by the user who submitted the transaction (e.g., on Ethereum there may be an expectation of ordering only by the sum of transaction's base fee and priority fee). This is despite the fact that such ordering contrary to user expectations may result in the transaction failing to execute successfully (despite being included in a block) or in the user realizing smaller economic value from the transaction than she would have in a different ordering (e.g. due to, respectively, "destructive" or "tolerating" front-running ~\cite{qin2022quantifying}).

\subsubsection{Our definitions}\label{sec:ourdef}
We begin by informally describing the ideal manner in which a blockchain transaction should execute when \emph{not} facing censorship.

\begin{definition}[Uncensored Transaction]\label{def:uncensoredTx}
Let's assume that a valid and signed user transaction is sent from a wallet to a blockchain infrastructure operator (such as a blockchain node). This operator and, if needed, other network participants (e.g., other node operators), forward the transaction within the network. Finally, the transaction reaches a blockchain operator (e.g., a validator), who includes it in a block, which in turn is added to the blockchain according to the underlying consensus mechanism. We consider the transaction to not be censored by any of the involved parties if the transaction's inclusion in the blockchain was not intentionally obstructed by any of them.
\end{definition}

This leads us to a definition of transaction censorship: Definition~\ref{def:censoredTx}.

\begin{definition}[Transaction Censorship]\label{def:censoredTx}
A transaction $tx$ is censored if its inclusion in a block is intentionally obstructed by any entity. If the obstruction is finite and $tx$ is eventually included in a block,  censorship is \emph{soft}. Otherwise, censorship is \emph{hard}.
\end{definition}

We note that the distinction between ``soft'' and ``hard'' censorship is made from the viewpoint of what eventually happens with the transaction, rather than from the perspective of what is achieved by any single censoring actor.

Definition~\ref{def:censoredTx} refers to intentional obstruction by ``any entity'', which may be interpreted narrowly, referring only to entities \emph{directly} obstructing a transaction, e.g., nodes that refuse to re-broadcast it or validators who refuse to include it in a block. In the empirical part of this paper, we adopt this narrow interpretation. However, a broad interpretation is also possible, referring also to entities \emph{indirectly} obstructing a transaction, e.g., a legal system that prohibits validators from including some transactions.

====
==== the stuff below is mostly unmodified compared to Aviv's version, until my added definition of "Censorship of a Node" and the content afterwards
====

The motivation for censoring a transaction may be in what it is meant to do, but also in what persons, bodies, or blockchain entities (smart contracts) are associated with that transaction. Thus, a transaction $tx$ could be censored due to a connection with a blockchain user who, e.g., is subject to legal sanctions, whether this user is a creator of $tx$, a recipient of funds transferred by $tx$, or is associated with any other entity which $tx$ interacts with, such as a smart contract which $tx$ invokes. Censorship against users could be tied to ephemeral and non-inherent features, like their country of residence.
In the context of a blockchain, one user might control multiple addresses which cannot be readily linked to each other~\cite{victor2020address,wang2022zero}, thereby leading those aiming to target users to focus on specific blockchain addresses~\cite{treasury2022cyber}.
Thus, we provide Definition~\ref{def:censoredAddress}, which distills the notion of censoring a blockchain address.

\begin{definition}[Address Censorship]\label{def:censoredAddress}
An address $\mathcal{A}$ is censored if a transaction involving $\mathcal{A}$ is censored per Definition~\ref{def:censoredTx}. Censorship is \emph{complete} in the time period $\mathcal{T}$ if all transactions involving $\mathcal{A}$ during $\mathcal{T}$ are censored, otherwise it is \emph{partial} during $\mathcal{T}$.
\end{definition}

Definition~\ref{def:censoredAddress} considers an address to be censored even if only a subset of the transactions interacting with it is censored. 
For example, in August of $2022$, \OFAC added the addresses of all Ethereum-deployed \TC smart contracts to its list of \SDN~\cite{treasury2022cyber}, thereby requiring the censorship of transactions interacting with these addresses by entities wanting to stay within the legal bounds of the United State's regulations. An unsanctioned user wishing to interact with \TC via a transaction would have this transaction censored by \OFAC-compliant actors, with the latter not applying any kind of censorship to transactions which solely interact with other unsanctioned entities.

In our blockchain system, transactions are included in blocks. Thus, in case a censored transaction (per Definition~\ref{def:censoredTx}) is included in a block, this can lead actors to censor the block, too. The decision of an actor to censor a block can also arise from other considerations, for example as a means to attack the system or to profit~\cite{apostolaki2017hijacking,yaish2022uncle}. Such considerations are generalized in Definition~\ref{def:censoredBlock}.


=====

=====


\item[Censorship of a Node:] A participant of a blockchain network (a node) may be blocked by other nodes (e.g. IP address-based refusal to peer) due to a legal obligation or for other reasons. A node's connection with the network may also be intentionally disrupted by actors external to the blockchain network (e.g., telecommunication service providers)~\cite{tran2020stealthier}.
\item[Censorship of a Blockchain:] Participation in and providing services (including telecommunication services) to a blockchain network may be legally prohibited in some jurisdictions. Such a prohibition may be enforced on the level of telecommunication services, e.g., BGP routing~\cite{tran2020stealthier}.
\end{description}

\textbf{\color{red}front-end censorship vs contract-based censorship.}


To add to related works:

\paragraph*{\bf Defining Censorship}
Related contexts in which ``censorship'' has been defined, at least indirectly (negatively), include works on censorship resistance (circumvention) in information systems in general~\cite{danezis2004economics,leberknight2010taxonomy,khattak2016sok,tschantz2016sok}, and works on censorship resistance of blockchains in particular~\cite{thin2018formal,zhang2019lay,xian2019improved,silva2020impact,crain2021red,}.
Our focus on selective censorship within a network (an information system), instead of censorship of entire networks is close to the concept of ``censorship susceptibility'' as defined by Perng, Reiter, and Wang~\cite{perng2005censorship}.



To add to references:

@inproceedings{perng2005censorship,
  title={Censorship resistance revisited},
  author={Perng, Ginger and Reiter, Michael K and Wang, Chenxi},
  booktitle={International Workshop on Information Hiding},
  pages={62--76},
  year={2005},
  organization={Springer}
}

@article{khattak2016sok,
  title={SOK: Making sense of censorship resistance systems},
  author={Khattak, Sheharbano and Elahi, Tariq and Simon, Laurent and Swanson, Colleen M and Murdoch, Steven J and Goldberg, Ian},
  journal={Proceedings on Privacy Enhancing Technologies},
  volume={2016},
  number={4},
  pages={37--61},
  year={2016}
}

@article{danezis2004economics,
  title={The economics of censorship resistance},
  author={Danezis, George and Anderson, Ross},
  journal={Proceedings of the 3rd Annual Workship on Economics and Information Security (WEIS04)(May 2004)},
  year={2004}
}

@inproceedings{tschantz2016sok,
  title={Sok: Towards grounding censorship circumvention in empiricism},
  author={Tschantz, Michael Carl and Afroz, Sadia and Paxson, Vern and others},
  booktitle={2016 IEEE Symposium on Security and Privacy (SP)},
  pages={914--933},
  year={2016},
  organization={IEEE}
}

@inproceedings{leberknight2010taxonomy,
  title={A taxonomy of Internet censorship and anti-censorship},
  author={Leberknight, Christopher S and Chiang, Mung and Poor, Harold Vincent and Wong, Felix},
  booktitle={Fifth International Conference on Fun with Algorithms},
  pages={52--64},
  year={2010}
}

@inproceedings{crain2021red,
  title={Red belly: a secure, fair and scalable open blockchain},
  author={Crain, Tyler and Natoli, Christopher and Gramoli, Vincent},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={466--483},
  year={2021},
  organization={IEEE}
}

@inproceedings{tran2020stealthier,
  title={A stealthier partitioning attack against bitcoin peer-to-peer network},
  author={Tran, Muoi and Choi, Inho and Moon, Gi Jun and Vu, Anh V and Kang, Min Suk},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={894--909},
  year={2020},
  organization={IEEE}
}

@inproceedings{silva2020impact,
  title={Impact of geo-distribution and mining pools on blockchains: A study of ethereum},
  author={Silva, Paulo and Vavricka, David and Barreto, Joao and Matos, Miguel},
  booktitle={2020 50th Annual IEEE/IFIP International Conference on Dependable Systems and Networks (DSN)},
  pages={245--252},
  year={2020},
  organization={IEEE}
}

@inproceedings{chitra2022improving,
  title={Improving Proof of Stake Economic Security via MEV Redistribution},
  author={Chitra, Tarun and Kulkarni, Kshitij},
  booktitle={Proceedings of the 2022 ACM CCS Workshop on Decentralized Finance and Security},
  pages={1--7},
  year={2022}
}

@techreport{auer2022miners,
  title={Miners as intermediaries: extractable value and market manipulation in crypto and DeFi},
  author={Auer, Raphael and Frost, Jon and Pastor, Jose Mar{\'\i}a Vidal and others},
  year={2022},
  institution={Bank for International Settlements}
}

@misc{buterin2021sok, title={State of research: Increasing censorship resistance of transactions under proposer/builder separation (PBS)}, url={https://notes.ethereum.org/@vbuterin/pbs_censorship_resistance}, journal={notes.ethereum.org}, author={Buterin, Vitalik}, year={2021}, month={Nov}}


@inproceedings{thin2018formal,
  title={Formal analysis of a proof-of-stake blockchain},
  author={Thin, Wai Yan Maung Maung and Dong, Naipeng and Bai, Guangdong and Dong, Jin Song},
  booktitle={2018 23rd International Conference on Engineering of Complex Computer Systems (ICECCS)},
  pages={197--200},
  year={2018},
  organization={IEEE}
}

@inproceedings{xian2019improved,
  title={Improved consensus mechanisms against censorship attacks},
  author={Xian, Xiangbin and Zhou, Yu and Guo, Yurong and Yang, Zhenguo and Liu, Wenyin},
  booktitle={2019 IEEE International Conference on Industrial Cyber Physical Systems (ICPS)},
  pages={718--723},
  year={2019},
  organization={IEEE}
}
